A Comprehensive and Modularized Statistical Framework for Gradient Norm Equality in Deep Neural Networks

In recent years, plenty of metrics have been proposed to identify networks that are free of gradient explosion and vanishing. However, due to the diversity of network components and complex serial-parallel hybrid connections in modern DNNs, the evaluation of existing metrics usually requires strong assumptions, complex statistical analysis, or has limited application fields, which constraints their spread in the community. In this paper, inspired by the Gradient Norm Equality and dynamical isometry, we first propose a novel metric called Block Dynamical Isometry, which measures the change of gradient norm in individual block. Because our Block Dynamical Isometry is norm-based, its evaluation needs weaker assumptions compared with the original dynamical isometry. To mitigate the challenging derivation, we propose a highly modularized statistical framework based on free probability. Our framework includes several key theorems to handle complex serial-parallel hybrid connections and a library to cover the diversity of network components. Besides, several sufficient prerequisites are provided. Powered by our metric and framework, we analyze extensive initialization, normalization, and network structures. We find that Gradient Norm Equality is a universal philosophy behind them. Then, we improve some existing methods based on our analysis, including an activation function selection strategy for initialization techniques, a new configuration for weight normalization, and a depth-aware way to derive coefficients in SeLU. Moreover, we propose a novel normalization technique named second moment normalization, which is theoretically 30% faster than batch normalization without accuracy loss. Last but not least, our conclusions and methods are evidenced by extensive experiments on multiple models over CIFAR10 and ImageNet.

==> algorithms/selu_res_alg.tex <==
\begin{algorithm}[ht]
\DontPrintSemicolon
 \KwData{the second order moment of input data: $m_2$; number of blocks: $L$; number of layers in one block: $m$; the standard deviation of weights: $\sqrt{\frac{\gamma}{n}}$; Factor $p$.}
 \KwResult{An $[L\times m, 2]$ matrix of the optimal $\lambda, \alpha$ for all the layers}
 \Begin{
 SeLU\_params = []\\
 \For{$l \in range(L)$}{
 $m_2^{(in)} = m_2$\\
 \For{$i \in range(m)$}{
 $[\lambda, \alpha] = solve$ \eqref{equ:solution_of_selu_resnet_fixup}$\backslash$ \eqref{equ:solution_of_selu_resnet}\\
 SeLU\_params.append($[\lambda, \alpha]$)\\
 $m_2 = $\eqref{equ:m2_selu_prop}[$m_2, \lambda, \alpha$]
 \;
 }
 $m_2 = m_2^{(in)} + m_2$\;
 }
 }
 \Return{SeLU\_params}
 \caption{SeLU for ResNet}
 \label{Alg:selu_res}
\end{algorithm}

==> chapters/pnasnet.tex <==
\subsection{NASNet}

For the normal cell, the input is 

\todo{----------------current progress------------}


To further demonstrate the effectiveness of our framework in the state-of-art network architectures, we investigate its application in the field of neural architecture search. We take the PNASNet proposed by Liu, Chenxi, et al.(2018)\cite{liu2018progressive} as demo, and explores whether it can be stabilized with other approaches beyond BN.


In PNASNet, a full CNN is constructed by stacking several ``cells" together. The basic unit in each cell is called ``blocks". The block $b$ of cell $c$ first individually applies transform, $O_1$ and $O_2$, to two input tensors, $I_1$ and $I_2$, respectively, then the results are combined with element-wise addition, the output is denoted as $H_b^{c}$. The output of a cell is the concatenation of the output of all its blocks. The input tensors are obtained from the set $\{H_1^c, H_2^c, ..., H_{b-1}^c\}\bigcup\{H_B^{c-1}, H_B^{c-2}\}$, $H_B^{c-1}$ and $H_B^{c-2}$ are the output of previous and previous-previous cells. The transform $O_i$ are chosen from a set of functions listed as follows.
\begin{itemize}
    \item $k\times k$ depthwise-separable convolution, $k\in\{3, 5, 7\}$.
    \item $1\times 7$ followed by $7\times 1$ convolution.
    \item identity.
    \item $3\times 3$ average/max pooling
    \item $3\times 3$ dilated convolution
\end{itemize}

\todo{Read the pytorch code to configure my understanding}




Ideas:
\begin{itemize}
    \item CNN is constructed by stacking cells together
    \item Each cell consists of several blocks, whereas the connection between blocks is complex. \item The analysis based on cell level is very complex, for there is dual connections between cells, and the connections within the cell is also complex. 
    \item Moreover, cell-level analysis is not suitable for the search progress, for it requires the handcrafted derivation even with our own framework
    \item Since the basic element of searching is block, which take a more regular structure and has fewer variants, as long as each block holds itself, the whole network will work (proof).
    \item But before our experiment, I believe we should mathematically model the whole searching space, configure the prerequisit, and prove that the stability of a PNASNet  
\end{itemize}



==> chapters/proofs/proof_LSTM.tex <==
\subsection{LSTM}
To begin with, we define
\begin{equation}
    \frac{\partial \mathbf{O}}{\partial \mathbf{X}} = {\left[\begin{array}{cccc}
    \frac{\partial \mathbf{o_1}}{\partial \mathbf{x_1}}&\frac{\partial \mathbf{o_1}}{\partial \mathbf{x_2}}&...&\frac{\partial \mathbf{o_1}}{\partial \mathbf{x_T}}\\
    \frac{\partial \mathbf{o_2}}{\partial \mathbf{x_1}}&\frac{\partial \mathbf{o_2}}{\partial \mathbf{x_2}}&...&\frac{\partial \mathbf{o_2}}{\partial \mathbf{x_T}}\\
    ...&...&&...\\
    \frac{\partial \mathbf{o_T}}{\partial \mathbf{x_1}}&\frac{\partial \mathbf{o_T}}{\partial \mathbf{x_2}}&...&\frac{\partial \mathbf{o_T}}{\partial \mathbf{x_T}}\\
\end{array}\right]} = {\left[\begin{array}{cccc}
    \mathbf{U_{1,1}}&\mathbf{U_{1,2}}&...&\mathbf{U_{1,T}}\\
    \mathbf{U_{2,1}}&\mathbf{U_{2,2}}&...&\mathbf{U_{2,T}}\\
    ...&...&&...\\
    \mathbf{U_{T,1}}&\mathbf{U_{T,2}}&...&\mathbf{U_{T,T}}\\
\end{array}\right]}
\end{equation}

According to \cite{hochreiter1997long},
\begin{equation}
    \begin{split}
        & \mathbf{f_t} = \sigma_f(\mathbf{W_fx_t} + \mathbf{U_fh_{t-1}} + \mathbf{b_f})\\
        & \mathbf{i_t} = \sigma_i(\mathbf{W_ix_t} + \mathbf{U_ih_{t-1}} + \mathbf{b_i})\\
        & \mathbf{o_t} = \sigma_o(\mathbf{W_ox_t} + \mathbf{U_oh_{t-1}}+\mathbf{b_o})\\
        & \mathbf{c_t} = \mathbf{f_t}\circ \mathbf{c_{t-1}} + \mathbf{i_t}\circ\sigma_c(\mathbf{W_cx_t} + \mathbf{U_ch_{t-1}} + \mathbf{b_c})\\
        & \mathbf{h_t} = \mathbf{o_t}\circ \sigma_h(\mathbf{c_t})
    \end{split}
\end{equation}

For $\mathbf{U_{p,q}}$, when $p<q$, as the state of the neuron at time $p$ is not affected by the state at time $q>p$, $\mathbf{U_{p,q}}=\mathbf{0}$; When $p=q$, $\mathbf{U_{p,q}}=\sigma_{g,p}'\mathbf{W_o}$, where $\sigma_{g,p}'$ denotes the jacobian matrix of activation function $\sigma_g$ with respect to the input of time $p$; When $p=q+k$:

\begin{equation}
\begin{split}
    &\frac{\partial \mathbf{o_p}}{\partial \mathbf{x_{p-k}}} = diag(\sigma_h(\mathbf{c_{p-1}}))\frac{\partial \mathbf{o_{p-1}}}{\partial \mathbf{x_{p-k}}} + diag(\mathbf{o_{p-1}})\sigma_{h,p-1}'\frac{\partial \mathbf{c_{p-1}}}{\partial \mathbf{x_{p-k}}}\\
    &\frac{\partial \mathbf{c_{p-1}}}{\partial \mathbf{x_{p-k}}} = diag(\mathbf{c_{p-2}})\frac{\partial \mathbf{f_{p-1}}}{\partial \mathbf{x_{p-k}}} + diag(\mathbf{f_{p-1}})\frac{\partial \mathbf{c_{p-2}}}{\partial \mathbf{x_{p-k}}} +\\
    & diag(\mathbf{i_{p-k}})\sigma_{c,p-1}(\mathbf{W_c}\frac{\partial \mathbf{x_{p-1}}}{\partial \mathbf{x_{p-k}}} + \mathbf{U_c}\frac{\partial \mathbf{h_{p-2}}}{\partial \mathbf{x_{p-k}}}) + diag(\sigma_c(\mathbf{W_cx_{p-1}} + \mathbf{U_ch_{p-2}} + \mathbf{b_c}))\frac{\partial \mathbf{i_{p-1}}}{\partial \mathbf{x_{p-k}}}\\
    &\frac{\partial \mathbf{f_{p-1}}}{\partial \mathbf{x_{p-k}}} = \sigma_{f,p-1}'(\mathbf{W_f}\frac{\partial \mathbf{x_{p-1}}}{\partial \mathbf{x_{p-k}}} + \mathbf{U_f}\frac{\partial \mathbf{h_{p-2}}}{\partial \mathbf{x_{p-k}}})\\
    & \frac{\partial \mathbf{i_{p-1}}}{\partial \mathbf{x_{p-k}}} = \sigma_{i,p-1}'(\mathbf{W_i}\frac{\partial \mathbf{x_{p-1}}}{\partial \mathbf{x_{p-k}}} + \mathbf{U_i}\frac{\partial \mathbf{h_{p-2}}}{\partial \mathbf{x_{p-k}}})\\
    & \frac{\partial \mathbf{h_{p-2}}}{\partial \mathbf{x_{p-k}}} = diag(\mathbf{o_{p-2}})\sigma_{h, p-2}'\frac{\partial \mathbf{c_{p-2}}}{\partial \mathbf{x_{p-k}}} + diag(\sigma_h(\mathbf{c_{p-2}}))\frac{\partial \mathbf{o_{p-2}}}{\partial \mathbf{x_{p-k}}})
\end{split}
\end{equation}

Our target is to evaluate $\phi(\frac{\partial \mathbf{O}}{\partial \mathbf{X}}^T\frac{\partial \mathbf{O}}{\partial \mathbf{X}})$. It's easy to see that
\begin{equation}
    \phi(\frac{\partial \mathbf{O}}{\partial \mathbf{X}}^T\frac{\partial \mathbf{O}}{\partial \mathbf{X}})=\frac{1}{T}\sum_{i=1}^T\sum_{j=1}^{i}\phi\left(\mathbf{U_{i,j}}^T\mathbf{U_{i,j}}\right)
\end{equation}

\todo{Prerequisites}

we have the recurrence formula

\todo{\rule[0pt]{0.6\textwidth}{0.05em}}\todo{Current Progress}



\begin{equation}
    \begin{split}
        &\mathbf{U}^{n,1}_{i,k} = \left[diag(f(\mathbf{o}^{i-1, n})) + diag(\mathbf{u}^{i-1, n})f_{i-1,n}'g_{i-1, n}'\right]\mathbf{U}^{n,1}_{i-1,k-1} + \mathbf{W_n}g_{i,n-1}'\mathbf{U}^{n-1,0}_{i, k}\\
        & \mathbf{U}^{n-1, 0}_{i,k} = g_{i,n-1}'\left[diag(\mathbf{u}^{i-1, n-1})f'_{i-1,n-1}g_{i-1,n-1}' + diag(f(\mathbf{o}^{i-1,n-1}))\right]\mathbf{U}_{i-1,k-1}^{n-1,0}
    \end{split}
\label{equ:lstm_recurrence_formula}
\end{equation}

Then we want to calculate 



With \eqref{equ:snn_recurrence_formula}, assuming that $\forall i,n$, 
\begin{equation}
\begin{split}
    &\mathbf{D}_{n,i} := \left[diag(f(\mathbf{o}^{i-1, n})) + diag(\mathbf{u}^{i-1, n})f_{i-1,n}'g_{i-1, n}'\right], \phi(\mathbf{D}_{n,i}^T\mathbf{D}_{n,i})=\mathbf{D}\\
    &\phi\left((g_{i,n-1})^Tg_{i,n-1}\right)=\mathbf{G}\\
    & \mathbf{Q}_{i,n} = g_{i,n-1}'\left[diag(\mathbf{u}^{i-1, n-1})f'_{i-1,n-1}g_{i-1,n-1}' + diag(f(\mathbf{o}^{i-1,n-1}))\right]\\ &\phi(\mathbf{Q}_{n,i}^T\mathbf{Q}_{n,i})=\mathbf{Q}
\end{split}
\end{equation}

we have the recurrence formula of $\phi$:
\begin{equation}
\begin{split}
    &\phi\left(\left(\mathbf{U}^{n,1}_{i,k}\right)^T\mathbf{U}^{n,1}_{i,k}\right) = \phi(\mathbf{D}^T\mathbf{D})\phi\left(\left(\mathbf{U}^{n,1}_{i-1,k-1}\right)^T\mathbf{U}^{n,1}_{i-1,k-1}\right)\\
    &+ \phi(\mathbf{W_n}^T\mathbf{W_n})\phi(\mathbf{G}^T\mathbf{G})\phi\left(\left(\mathbf{U}^{n-1,0}_{i,k}\right)^T\mathbf{U}^{n-1,0}_{i,k}\right)\\
    &\phi\left(\left(\mathbf{U}^{n-1,0}_{i,k}\right)^T\mathbf{U}^{n-1,0}_{i,k}\right) = \phi(\mathbf{Q}^T\mathbf{Q})\phi\left(\left(\mathbf{U}^{n-1,0}_{i-1,k-1}\right)^T\mathbf{U}^{n-1,0}_{i-1,k-1}\right)
\end{split}
\end{equation}





==> chapters/proofs/proof_SNN.tex <==
\subsection{Spiking Neural Network}
To begin with, we denote $\mathbf{U}_{i,k}^{n,1} := \frac{\partial \mathbf{u}^{i,n}}{\partial \mathbf{o}^{i-k, n-1}}$, $\mathbf{U}_{i,k}^{n,0} := \frac{\partial \mathbf{u}^{i,n}}{\partial \mathbf{o}^{i-k, n}}$, and we define
\begin{equation}
    \frac{\partial \mathbf{U}^n}{\partial \mathbf{O}^{n-1}} = {\left[\begin{array}{cccc}
    \frac{\partial \mathbf{u}^{1,n}}{\partial \mathbf{o}^{1, n-1}}&\frac{\partial \mathbf{u}^{1,n}}{\partial \mathbf{o}^{2, n-1}}&...&\frac{\partial \mathbf{u}^{1,n}}{\partial \mathbf{o}^{T, n-1}}\\
    \frac{\partial \mathbf{u}^{2,n}}{\partial \mathbf{o}^{1, n-1}}&\frac{\partial \mathbf{u}^{2,n}}{\partial \mathbf{o}^{2, n-1}}&...&\frac{\partial \mathbf{u}^{2,n}}{\partial \mathbf{o}^{T, n-1}}\\
    ...&...&&...\\
    \frac{\partial \mathbf{u}^{T,n}}{\partial \mathbf{o}^{1, n-1}}&\frac{\partial \mathbf{u}^{T,n}}{\partial \mathbf{o}^{2, n-1}}&...&\frac{\partial \mathbf{u}^{T,n}}{\partial \mathbf{o}^{T, n-1}}
\end{array}\right]} = {\left[\begin{array}{cccc}
    \mathbf{U}^{n,1}_{1,0}&\mathbf{U}^{n,1}_{1,-1}&...&\mathbf{U}^{n,1}_{1,-T+1}\\
    \mathbf{U}^{n,1}_{2,1}&\mathbf{U}^{n,1}_{2,0}&...&\mathbf{U}^{n,1}_{2,-T+2}\\
    ...&...&&...\\
    \mathbf{U}^{n,1}_{T,T-1}&\mathbf{U}^{n,1}_{T,T-2}&...&\mathbf{U}^{n,1}_{T,0}
\end{array}\right]}
\end{equation}

According to \cite{wu2018spatio},
\begin{equation}
    \begin{split}
        & \mathbf{o}^{t, n} = g(\mathbf{u}^{t, n}),~~g(x) = 1~~if~~x\ge V_{th} ~~else~~ 0\\
        & \mathbf{u}^{t, n} = f(\mathbf{o}^{t-1, n})\circ \mathbf{u}^{t-1, n} + \mathbf{W}_{n}\mathbf{o}^{t, n-1} + \mathbf{b}^n,~~f(x) = \tau e^{-\frac{x}{\tau}},~~\mathbf{u}^{0,n}=\mathbf{u}^{0,n-1}=\mathbf{0}
    \end{split}
\end{equation}

$\forall n$, when $k<0$, As the state of the neuron at time $i$ is not affected by the state at time $j>i$, $\mathbf{U}_{i,k<0}^{n,1}=\mathbf{U}_{i,k<0}^{n,0}=\mathbf{0}$; When $k=0$, we have $\mathbf{U}_{i,0}^{n,1}=\mathbf{W_n}$, $\mathbf{U}_{i,0}^{n,0}=\mathbf{0}$; When $k>0$,

\begin{equation}
\begin{split}
    & \frac{\partial \mathbf{u}^{i,n}}{\partial \mathbf{o}^{i-k, n-1}} = diag(f(\mathbf{o}^{i-1, n})) \frac{\partial \mathbf{u}^{i-1,n}}{\partial \mathbf{o}^{i-k, n-1}} + diag(\mathbf{u}^{i-1, n})f_{i-1,n}'\frac{\partial \mathbf{o}^{i-1,n}}{\partial \mathbf{o}^{i-k, n-1}}  + \mathbf{W}_n\frac{\partial \mathbf{o}^{i,n-1}}{\partial \mathbf{o}^{i-k, n-1}}
\end{split}
\end{equation}
As
\begin{equation}
\begin{split}
    &\frac{\partial \mathbf{u}^{i-1,n}}{\partial \mathbf{o}^{i-k, n-1}} = \frac{\partial \mathbf{u}^{i-1,n}}{\partial \mathbf{o}^{(i-1)-(k-1), n-1}} = \mathbf{U}_{i-1, k-1}^{n,1},~~\frac{\partial \mathbf{o}^{i-1,n}}{\partial \mathbf{o}^{k-1, n-1}}=g_{i-1,n}'\mathbf{U}_{i-1, k-1}^{n,1}\\
    & \frac{\partial \mathbf{o}^{i,n-1}}{\partial \mathbf{o}^{i-k, n-1}} = g'_{i, n-1}\left[diag(\mathbf{u}^{i-1, n-1})f'_{i-1,n-1}\frac{\partial \mathbf{o}^{i-1,n-1}}{\partial \mathbf{o}^{i-k, n-1}} + diag(f(\mathbf{o}^{i-1,n-1}))\frac{\partial \mathbf{u}^{i-1,n-1}}{\partial \mathbf{o}^{i-k, n-1}}\right]\\
    & = g'_{i, n-1}\left[diag(\mathbf{u}^{i-1, n-1})f'_{i-1,n-1}g_{i-1,n-1}'\mathbf{U}_{i-1,k-1}^{n-1,0} + diag(f(\mathbf{o}^{i-1,n-1}))\mathbf{U}_{i-1,k-1}^{n-1,0}\right]
\end{split}
\end{equation}

we have the recurrence formula
\begin{equation}
    \begin{split}
        &\mathbf{U}^{n,1}_{i,k} = \left[diag(f(\mathbf{o}^{i-1, n})) + diag(\mathbf{u}^{i-1, n})f_{i-1,n}'g_{i-1, n}'\right]\mathbf{U}^{n,1}_{i-1,k-1} + \mathbf{W_n}g_{i,n-1}'\mathbf{U}^{n-1,0}_{i, k}\\
        & \mathbf{U}^{n-1, 0}_{i,k} = g_{i,n-1}'\left[diag(\mathbf{u}^{i-1, n-1})f'_{i-1,n-1}g_{i-1,n-1}' + diag(f(\mathbf{o}^{i-1,n-1}))\right]\mathbf{U}_{i-1,k-1}^{n-1,0}
    \end{split}
\label{equ:snn_recurrence_formula}
\end{equation}

Then we want to calculate $\phi(\frac{\partial \mathbf{U}^n}{\partial \mathbf{O}^{n-1}}^T\frac{\partial \mathbf{U}^n}{\partial \mathbf{O}^{n-1}})$. It's easy to see that
\begin{equation}
    \phi\left(\frac{\partial \mathbf{U}^n}{\partial \mathbf{O}^{n-1}}^T\frac{\partial \mathbf{U}^n}{\partial \mathbf{O}^{n-1}}\right)=\frac{1}{T}\sum_{i=1}^T\sum_{j=1}^{i}\phi\left(\left(\mathbf{U}^{n,1}_{i, i-j}\right)^T\mathbf{U}^{n,1}_{i, i-j}\right)
\end{equation}

\todo{Prerequisites}

With \eqref{equ:snn_recurrence_formula}, assuming that $\forall i,n$, 
\begin{equation}
\begin{split}
    &\mathbf{D}_{n,i} := \left[diag(f(\mathbf{o}^{i-1, n})) + diag(\mathbf{u}^{i-1, n})f_{i-1,n}'g_{i-1, n}'\right], \phi(\mathbf{D}_{n,i}^T\mathbf{D}_{n,i})=\mathbf{D}\\
    &\phi\left((g_{i,n-1})^Tg_{i,n-1}\right)=\mathbf{G}\\
    & \mathbf{Q}_{i,n} = g_{i,n-1}'\left[diag(\mathbf{u}^{i-1, n-1})f'_{i-1,n-1}g_{i-1,n-1}' + diag(f(\mathbf{o}^{i-1,n-1}))\right]\\ &\phi(\mathbf{Q}_{n,i}^T\mathbf{Q}_{n,i})=\mathbf{Q}
\end{split}
\end{equation}

we have the recurrence formula of $\phi$:
\begin{equation}
\begin{split}
    &\phi\left(\left(\mathbf{U}^{n,1}_{i,k}\right)^T\mathbf{U}^{n,1}_{i,k}\right) = \phi(\mathbf{D}^T\mathbf{D})\phi\left(\left(\mathbf{U}^{n,1}_{i-1,k-1}\right)^T\mathbf{U}^{n,1}_{i-1,k-1}\right)\\
    &+ \phi(\mathbf{W_n}^T\mathbf{W_n})\phi(\mathbf{G}^T\mathbf{G})\phi\left(\left(\mathbf{U}^{n-1,0}_{i,k}\right)^T\mathbf{U}^{n-1,0}_{i,k}\right)\\
    &\phi\left(\left(\mathbf{U}^{n-1,0}_{i,k}\right)^T\mathbf{U}^{n-1,0}_{i,k}\right) = \phi(\mathbf{Q}^T\mathbf{Q})\phi\left(\left(\mathbf{U}^{n-1,0}_{i-1,k-1}\right)^T\mathbf{U}^{n-1,0}_{i-1,k-1}\right)
\end{split}
\end{equation}

\todo{\rule[0pt]{0.6\textwidth}{0.05em}}\todo{Current Progress}



==> chapters/selu_stabilizer.tex <==








==> chapters/sketch.tex <==
Given dynamic system defined as:
\begin{equation}
    y'(t) = f(t, y(t)), ~~, t\ge 0, ~~y(t_0) = y_0
\label{equ:stable_ode}
\end{equation}
As argued in \cite{chen2018neural}, a neural network can be seen as a Euler 
If $y_0$ changes by a little factor $\delta_0$
\begin{equation}
    (y+\delta(t))' = f(t, y(t)+\delta(t)), ~~, t\ge 0, ~~y(t_0) = y_0+\delta_0
\label{equ:stable_ode_delta}
\end{equation}
Assuming that $t-t_0$ and $\delta_0$ are sufficiently small, \eqref{equ:stable_ode} - \eqref{equ:stable_ode_delta} can be expanded about $(t_0, y_0)$:
\begin{equation}
        \delta'(t)\approx f_y(t_0, y_0)\delta(t) = \lambda\delta(t)
\label{equ:ode_delta}
\end{equation}
where $\lambda=f_y(t_0,y_0)$. The solution of \eqref{equ:ode_delta} is
\begin{equation}
    \delta(t) = \delta_0e^{\lambda t}
\label{equ:ode_delta_solution}
\end{equation}

For a system defined by a set of ODE, \eqref{equ:ode_delta} can be rewritten as:
\begin{equation}
    \mathbf{\delta}'(t)\approx \mathbf{\Lambda\delta}(t)
\label{equ:vector_ode_delta}
\end{equation}
$\mathbf{\Lambda}$ is the Jacobian matrix defined as $[\mathbf{f}_y(t, \mathbf{y})]_{i, j} = \frac{\partial f_i}{\partial y_j}$. In many cases, $\mathbf{\Lambda}$ can be break down into $P^{-1}DP$, and \eqref{equ:vector_ode_delta} can be break down into a set of ODEs that are equivalent with \eqref{equ:ode_delta}
\begin{equation}
    z'_i = \lambda_iz
\end{equation}

with $\lambda_1,...\lambda_n$ the eigenvalues of $\mathbf{\Lambda}$.

For a neural network trained for supervised classification system, we say it is stable if and only if it can tolerant small differences between datas that share the same category while reserve the gap between datas of different categories.

By modeling the neural network as a dynamic system, we can see that the propagation of the initial difference of datas can be modeled by \eqref{equ:ode_delta_solution}. Since $\lambda$ can be a complex number, it's obviously that with a large $Re(\lambda)$, the difference would scale exponentially, which results in an unstable network. Similarly, if the $Re(\lambda)$ is a huge negative value, even a huge initial difference would be decayed exponentially.

Notably, when the input data is described as a vector, the $\lambda$ are the eigenvalues of its Jacobian matrix, and the network is well-posed and stable if
\begin{equation}
    |Re(\lambda_i(\mathbf{\Lambda}))| < \epsilon, ~~\forall t\in [0, 1], ~~i=1,2..,n
\label{equ:stable&well_posed}
\end{equation}
This accords with the conclusions of \cite{haber2017stable}.

\todo{stability of Euler system}

\begin{comment}

For the ResNet Block with single layer modeled as $\mathbf{y}_{t+1} = \mathbf{y}_t + relu(norm(\mathbf{K}_t\mathbf{y}_t))$. The input  $\mathbf{y}_t \in \mathbb{R}^n$ is initialized by: $\forall i \in [0, n),~~ [\mathbf{y}_t]_i \sim max(0, N(0, \nu))$ as it is activated by relu in the previous layer. During the training, the parameters in $\mathbf{K}_t$ is being updated, so we initialize it by: $\forall i,j\in[0, n), ~~[\mathbf{K}_t]_{i, j} \sim N(\mu, \sigma^2)$. We evaluate the $E(max|1+Re(eig(\mathbf{f_y}))|)$ and $E(mean|1+Re(eig(\mathbf{f_y}))|)$ under different domains of $(\nu, \mu, \sigma)$ and see if conjecture 1 is satisfied. The expectation is calculated by taking the mean of 200 independent experiments.

\begin{figure}[h]
\centering
\includegraphics[width=0.95\textwidth]{figure/eig_K_bn.pdf}
\caption{Left: experiment of ResNet on domain $(\nu=1, \mu=0, \sigma \in [0.1, 2.0])$; Right: experiment of ResNet on domain $(\nu=1, \mu \in [-0.2, 0.2], \sigma=1)$}
\label{fig:eig_K_bn}
\end{figure}

Fig. \ref{fig:eig_K_bn} illustrate that $E(mean|1+Re(eig(\mathbf{f_y}))|)$ and $E(max|1+Re(eig(\mathbf{f_y}))|)$ of normalized network is unaffected by the shifting or scaling of the weight matrix, which accords with the conclusions of \cite{ioffe2015batch}. Although the maximum 2 is a little higher, we will illustrate later that it would decay to $1^+$ when the network goes deeper.

The Resnet block is defined as $\mathbf{y}_{t+1} = \mathbf{y}_{t} + \mathbf{f}(\mathbf{y}_t)$. Assuming that $\forall i,~[\mathbf{y}_t]_i \in N(0, \nu_t)$ and $\mathbf{f}(\mathbf{y}_t)$ independents with $\mathbf{y}_t$, for the reason that the output of $\mathbf{f}$ is normalized, $\forall i,~[\mathbf{f}(\mathbf{y}_t)]_i \in N(0, 1)$. It's easy to derive that $\nu_{t+1} = \sqrt{1+\nu_t^2}$. Fig. \ref{fig:eig_y_bn} (left) illustrate how $\nu$ scales up when the network goes deeper, and Fig. \ref{fig:eig_y_bn} (right) shows that the $E(max|1+Re(eig(\mathbf{f_y}))|)$ would converges to $1^+$ when $\nu$ gets larger. As a result, ResNet perfectly satisfies conjecture 1, which explains ResNet's superior.

\begin{figure}[h]
\centering
\includegraphics[width=0.95\textwidth]{figure/eig_y_bn.pdf}
\caption{Left: the scaling up of $\nu$ when the network goes deeper; Right: experiment of ResNet on domain $(\nu \in [0.1, 5], \mu = 0, \sigma=1)$}
\label{fig:eig_y_bn}
\end{figure}

We also test the conjecture 1 on vanilla network, as shown in Fig. \ref{fig:eig_K_bn_v}. It's obviously that 1). BN successfully stabilizes $E(mean|1+Re(eig(\mathbf{f_y}))|)$ and $E(max|1+Re(eig(\mathbf{f_y}))|)$; 2). $E(max|1+Re(eig(\mathbf{f_y}))|) \approx 1$, which indicates that all the differences are getting decayed during their propagation, thus vanilla networks cannot go very deep.

\begin{figure}[h]
\centering
\includegraphics[width=0.95\textwidth]{figure/eig_K_bn_v.pdf}
\caption{Left: experiment of vanilla network on domain $(\nu=1, \mu=0, \sigma \in [0.1, 2.0])$; Right: experiment of vanilla network on domain $(\nu=1, \mu \in [-0.2, 0.2], \sigma=1)$}
\label{fig:eig_K_bn_v}
\end{figure}

Another interesting discovery of Fig. \ref{fig:eig_y_bn} (right) is that the curve "norm max" perfectly fits the curve "$1+1/\nu$". Inspired by this, we make the following conjecture:

\textit{\textbf{Conjecture 2}. For a random vectors $\mathbf{x}\in \mathbb{R}^n$, we define a function $f(\cdot, \mathbf{\omega})$ that maps $\mathbf{x}$ to $\mathbf{y} \in \mathbb{R}^n$: $\mathbf{y} = f(\mathbf{x}, \mathbf{\omega})$, $\mathbf{\omega}$ is also a random variable.}

\textit{Assuming that $f(\cdot, \mathbf{\omega})$ satisfies $\forall \mathbf{x}, \alpha std(\mathbf{y}) = std(\mathbf{x})$. Then we have $E(max(|Re(\frac{\partial \mathbf{f}}{\partial \mathbf{x}})|)) = 1 / \alpha$.}


\subsection{Backward Pass}
\todo{Backward Pass: The stability of the backward pass can be analysed from the stability of the backward ODE function proposed by \cite{chen2018neural}.}
\begin{comment}
\cite{chen2018neural} provides a way to perform backpropagation through a ODE Solver. For a forward pass formulated as 
\begin{equation}
    \frac{d\mathbf{h}(t)}{dt} = f(\mathbf{h}(t), t, \theta)
\end{equation}
It's corresponding backward pass can be solved with a set of ODEs
\begin{equation}
    \begin{split}
        &\frac{d \mathbf{\alpha}(t)}{dt} = -\mathbf{\alpha}(t)^T\frac{\partial \mathbf{f}(\mathbf{h}(t), t, \theta)}{\partial \mathbf{h}},~~\mathbf{\alpha}(t) = \frac{\partial L}{\partial \mathbf{h}(t)}\\
        &\frac{d \mathbf{\alpha}_{\theta}(t)}{dt} = -\mathbf{\alpha}(t)^T\frac{\partial \mathbf{f}(\mathbf{h}(t), t, \theta)}{\partial \theta}, ~~\mathbf{\alpha}_{\theta}(t) = \frac{\partial L}{\partial \theta}
    \end{split}
\label{equ:ODE_backward}
\end{equation}
In our case, solving \eqref{equ:BN_ODE_forward} following \eqref{equ:ODE_backward} can be written as:
\begin{equation}
    \begin{split}
        &\frac{d \mathbf{\alpha}(t)}{dt} = -\mathbf{\alpha}(t)^T\frac{\partial \mathbf{f}(\mathbf{y}(t), t, \mathbf{K}^T)}{\partial \mathbf{y}},~~\mathbf{\alpha}(t) = \frac{\partial L}{\partial \mathbf{h}(t)}\\
        &\frac{d \mathbf{\alpha}_{\theta}(t)}{dt} = -\mathbf{\alpha}(t)^T\frac{\partial \mathbf{f}(\mathbf{y}(t), t, \mathbf{K}^T)}{\partial \mathbf{K}^T}, ~~\mathbf{\alpha}_{\theta}(t) = \frac{\partial L}{\partial \mathbf{K}^T}
    \end{split}
\label{equ:BN_ODE_backward}
\end{equation}
\eqref{equ:BN_ODE_backward} can be reformulated following \eqref{equ:calculate_JM_0}
\begin{equation}
    \begin{split}
        &\frac{d \mathbf{\alpha}(t)}{dt} = -\mathbf{\alpha}(t)^T\times\mathbf{f_g}\times\mathbf{g_u}\times\mathbf{u_y},~~\mathbf{\alpha}(t) = \frac{\partial L}{\partial \mathbf{h}(t)}\\
        &\frac{d \mathbf{\alpha}_{\theta}(t)}{dt} = -\mathbf{\alpha}(t)^TT\times\mathbf{f_g}\times\mathbf{g_u}\times\mathbf{u_{K^T}}, ~~\mathbf{\alpha}_{\theta}(t) = \frac{\partial L}{\partial \mathbf{K}^T}
    \end{split}
\label{equ:BN_ODE_backward_2}
\end{equation}
According to \eqref{equ:stable&well_posed}, \eqref{equ:BN_ODE_backward_2} is stable and well-posed as long as it satisfies:
\end{comment}

\end{comment}

\subsection{batch normalization based residual network}
The major challenge that the shortcut brings is that it breaks down the jacobian matrix into several parts that are non-hermitian and not freely independent with each other. For instance, letting the jacobian matrix of a residual layer to be $\hat{\mathbf{J}} = (\mathbf{I} + \mathbf{J})$:
\begin{equation}
    \hat{\mathbf{J}}\hat{\mathbf{J}}^T = \mathbf{I} + \mathbf{J} + \mathbf{J}^T + \mathbf{JJ}^T
\end{equation}
\cite{ling2018spectrum} analyzes the "without BN" version of fully-connected ResNet with the tools of non-Hermitian free probability:

\textit{
(The distribution of eigenvalues of single residual layer without BN) \citep{ling2018spectrum} for a layer whose input-output jacobian matrix denoted as $\mathbf{J}:=\mathbf{I}+\mathbf{D}\mathbf{K}$, where $\mathbf{D}$ is the jacobian of relu and $[\mathbf{K}\in\mathbb{R}^{m\times m}]_{i,j}\sim N(0, \sigma_K^2)$. Thus the S-transform of the distribution of eigenvalues in $\mathbf{DD}^T,\mathbf{KK}^T$ are $S_{\mathbf{DD}^T(z)}=\frac{z+1}{z+p}$ and $S_{\mathbf{KK}^T}(z)=\frac{1}{m\sigma_K^2(z+1)}$, respectively. Then, }
\begin{equation}
    \mu_{\mathbf{JJ}^T}=1+\sigma_K^2mp,~~\sigma_{\mathbf{JJ}^T}=\sigma_K^2mp(2+m\sigma_K^2)
\label{equ:spectrum:conclusion}
\end{equation}

Following \cite{ling2018spectrum}'s derivation, we analyze the residual layer where BN is applied.

With \eqref{equ:bn_eig_expansion} and \textit{\textbf{lemma 1}}, the eigenvalues of $\mathbf{g_ug_u}^T$ are:
\begin{equation}
    \lim_{m\rightarrow\infty}[\lambda_{\mathbf{g_ug_u}^T}]_i = \frac{1}{\sigma_B^2}\left\{
             \begin{array}{lr}
             0~~~~~~i=1,2\\
             1~~~~~~else
             \end{array}
\right.
\end{equation}
and the spectral density of $\mathbf{g_ug_u}^T$ can be written as:
\begin{equation}
    \rho_{\mathbf{g_ug_u}^T}(\lambda) = \frac{2}{m}\delta(\lambda)+(1-\frac{2}{m})\delta(\lambda-\frac{1}{\sigma_B^2}) \approx \delta(\lambda-\frac{1}{\sigma_B^2})
\end{equation}
Following \eqref{equ:stieltjes transform}, \eqref{equ:M-transform} and \eqref{equ:S-transform}, we can derive the S-transform of $\rho_{\mathbf{g_ug_u}^T}(\lambda)$:
\begin{equation}
    \begin{split}
        &G_{\mathbf{g_ug_u}^T}(z) = \int_{\mathbb{R}}\frac{\delta(t-\frac{1}{\sigma_B^2})}{z-t}dt = \frac{1}{z-\frac{1}{\sigma_B^2}}\\
        &M_{\mathbf{g_ug_u}^T}(z) = zG_{\mathbf{g_ug_u}^T}-1=\frac{\frac{1}{\sigma_B^2}}{z-\frac{1}{\sigma_B^2}}\\
        &M^{-1}_{\mathbf{g_ug_u}^T}(z)=\frac{1}{\sigma_B^2}(1+\frac{1}{z}),~~S_{\mathbf{g_ug_u}^T}(z)=\sigma_B^2
    \end{split}
\end{equation}

With BN, the jacobian matrix is $\mathbf{J}:=\mathbf{I}+\mathbf{f_gg_uu_y}$, \todo{proof:freely independent}, with the property of S-transform:
\begin{equation}
    S_{\mathbf{f_gg_uu_yu_y}^T\mathbf{g_u}^T\mathbf{f_g}^T} = S_{\mathbf{f_gf_g}^T}S_{\mathbf{g_ug_u}^T}S_{\mathbf{u_yu_y}^T}=\frac{\sigma_B^2}{m\sigma_K^2(z+p)} = \frac{1}{m\hat{\sigma_K}^2(z+p)}
\end{equation}
where$\hat{\sigma_w}=\frac{\sigma_w}{\sigma_B}$. As a result, with the conclusion of \eqref{equ:spectrum:conclusion}, we have the 
\begin{equation}
    \E[eig(\mathbf{JJ}^T)]=1+\sigma_K^2/\sigma_B^2mp,~~D[eig(\mathbf{JJ}^T)]=\sigma_K^2/\sigma_B^2mp(2+m\sigma_K^2/\sigma_B^2)
\label{equ:bn_resnet_conclusion}
\end{equation}

\eqref{equ:bn_resnet_conclusion} illustrates that when mean of the weight kernel is $0$, BN actually acts like a normalization of the weight kernel.

\begin{comment}
To sum up, \eqref{equ:the_forge} and \eqref{equ:the_forge_add} illustrates that when evaluating the neural network with both series and parallel connections, the metrics of \eqref{equ:target_E} and \eqref{equ:target_V} can be easily derived from the metrics of each network's component.

\subsection{Limitations}
The prelimitation for \eqref{equ:the_forge} is that the involved random matrices should be asymptotically free, which is the foundation of free probability. 

A basic observation of asymptotically free made by Voiculescu in 1991 \citep{voiculescu1991limit} suggests that:

\textit{Consider $N\times N$ random matrices $\mathbf{X_N}$ and $\mathbf{Y_N}$ such that: both $\mathbf{X_N}$ and $\mathbf{Y_N}$ have almost surely an asymptotic eigenvalue distribution for $N\rightarrow\infty$; $\mathbf{X_N}$ and $\mathbf{Y_N}$ are independent; $\mathbf{Y_N}$ is a unitary invariant ensemble (i.e., the joint distribution of its entries does not change under unitary conjugation, thus for any unitary $N\times N$-matrix $\mathbf{U_N}$, $\mathbf{U_NY_NU_N}^*$ is equivalent to the original ensemble $\mathbf{Y_N}$ in all relevant aspects). Then, $\mathbf{X_N}$ and $\mathbf{Y_N}$ are almost surely asymptotically free.}

Assuming that for the weight kernel $\mathbf{K}$ of a fully-connected layer, all the entries $k_{i,j}:=[\mathbf{K}]_{i,j}$ are i.i.d. As the unitary transformation preserves the l2-norm, as long as the expectation of the the entries doesn't change, with the central limit theorem, $K$ would be a unitary invariant ensemble.Given a unitary matrix $[\mathbf{U}]_{i,j} = u_{i, j}$, the expectation of entry $\hat{k}_{i,j}$ of $\mathbf{UKU}^*$ is:
\begin{equation}
    E[\hat{k}_{i,j}] = E[k_{i,j}]\sum_{p=1}^N\sum_{q=1}^Nu_{i,q}u_{j,p}^*
\end{equation}
As there is no guarantee that $\sum_{p=1}^N\sum_{q=1}^Nu_{i,q}u_{j,p}^*\equiv1$, we have to force $E[\hat{k}_{i,j}]\equiv0$.

Fortunately, this is not a strong assumption, which is almost held in neural networks. Moreover, it brings several conveniences: 1). for any random $N\times N$ matrix $\mathbf{A}$ that is independent with $\mathbf{K}$, $E[\mathbf{AK}]_{i,j}\equiv0$, and thus $\mathbf{AK}$ is also a unitary invariant ensemble. 2). For any unitary matrix $mathbf{U}$, $\mathbf{UKK}^T\mathbf{U}^*=\mathbf{UKU}^*\mathbf{UK}^T\mathbf{U}^* = \mathbf{KK}^T$, thus $\mathbf{KK}^T$ is also a unitary invariant ensemble.
\end{comment}



\begin{comment}
\subsection{Challenges}\label{sec:challenges}
In both \eqref{equ:forward_expect_l2_norm} and \eqref{equ:backward_expect_l2_norm}, we have to calculate a term which takes the form of $\phi\left(\left(\Pi_{i}\mathbf{J_i})(\Pi_{i}\mathbf{J_i}\right)^T\right)$, where $\mathbf{J_i}$s are random matrices. Notably, each $\mathbf{J_i}$ might also be the multiplication or summation of some random matrices. 

For instance, consider a ResNet for which each $\mathbf{J_i}$ denotes the input-output jacobian matrix of a residual block illustrated in Fig. \ref{fig:simple_res_block}.
\begin{figure}[ht]
\centering
\includegraphics[width=0.7\textwidth]{figure/resblock.pdf}
\caption{Simple Residual Block}
\label{fig:simple_res_block}
\end{figure}

With the chain law, we have:
\begin{equation}
\begin{split}
    & \mathbf{y} = \mathbf{x} + BN_2\circ CONV_2\circ ReLU_2\circ BN_1\circ CONV_1\circ ReLU_1(\mathbf{x})\\
    & \mathbf{J_i} = \mathbf{I} + \mathbf{J_{BN_2}J_{CONV_2}J_{ReLU_2}J_{BN_1}J_{CONV_1}J_{ReLU_2}}
\end{split}
\end{equation}
where $\mathbf{J_{X}}$ denotes the corresponding input-output jacobian matrix of Operator $X$. As $\mathbf{J_{X}}$s are random matrices with different statistics properties, even $\phi(\mathbf{J_i}\mathbf{J_i}^T)$ is challenging enough, not to mention $\phi\left(\left(\Pi_{i}\mathbf{J_i})(\Pi_{i}\mathbf{J_i}\right)^T\right)$.
\end{comment}

\begin{comment}
We denote $\mathbf{J_{L\rightarrow i+1}}:=\Pi_{j=L}^{i+1}\mathbf{J_j}$, $\Delta \mathbf{\theta_i}:=- \eta \left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)^T\left(\mathbf{J_{L\rightarrow i+1}}\right)^T \frac{\partial}{\partial f(\mathbf{x})}\mathcal{L}(f(\mathbf{x}), \mathbf{y})$, and 
\begin{equation}
    ||\Delta \theta_i||_2^2 = \eta^2 \left(\frac{\partial}{\partial f(\mathbf{x})}\mathcal{L}(f(\mathbf{x}), \mathbf{y})\right)^T\left(\mathbf{J_{L\rightarrow i+1}}\right)\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)^T\left(\mathbf{J_{L\rightarrow i+1}}\right)^T\frac{\partial}{\partial f(\mathbf{x})}\mathcal{L}(f(\mathbf{x}), \mathbf{y})
\end{equation}
which can be represented as quadratic form: $\alpha_2(\Delta \theta_i) = \mathbf{x}^T\mathbf{Q\Lambda Q}^T\mathbf{x}$, where $\mathbf{Q\Lambda Q}^T := \left(\mathbf{J_{L\rightarrow i+1}}\right)\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)^T\left(\mathbf{J_{L\rightarrow i+1}}\right)^T$, $\mathbf{x}:=\frac{\partial}{\partial f(\mathbf{x})}\mathcal{L}(f(\mathbf{x})$ and $\mathbf{Q}$ is a unitary matrix. In order to compute the expectation of $\alpha_2(\Delta \theta_i)$, we make two assumptions:
\begin{itemize}
    \item $\forall i,j, E[\mathbf{x}_i^2] = E[\mathbf{x}_j^2]$
    \item $\left(\mathbf{J_{L\rightarrow i+1}}\right)^T\left(\mathbf{J_{L\rightarrow i+1}}\right)$ is freely independent with $\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)^T$
\end{itemize}
Under these assumptions, with \eqref{equ:the_forge}, we have:
\begin{equation}
    E[\alpha_2(\Delta \theta_i)] = E\left[\alpha_2\left(\mathbf{x}\right)\right]E\left[tr\left(\left(\mathbf{J_{L\rightarrow i+1}}\right)^T\left(\mathbf{J_{L\rightarrow i+1}}\right)\right)\right]E\left[tr\left(\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)^T\right)\right]
\end{equation}
We can see that as long as $E\left[\alpha_2\left(\mathbf{x}\right)\right]$ and $E\left[tr\left(\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)\left(\frac{\partial f_{i}}{\partial \mathbf{\theta_{i}}}\right)^T\right)\right]$ has limited value (the forward pass doesn't explode or vanish), $E[\alpha_2(\Delta \theta_i)] \propto E\left[eig\left(\left(\mathbf{J_{L\rightarrow i+1}}\right)\left(\mathbf{J_{L\rightarrow i+1}}\right)^T\right)\right]$.

Again, with \eqref{equ:the_forge}, $E\left[eig\left(\left(\mathbf{J_{L\rightarrow i+1}}\right)\left(\mathbf{J_{L\rightarrow i+1}}\right)^T\right)\right] = \Pi_{j=i+1}^L E\left[eig\left(\left(\mathbf{J_j}\mathbf{J_j}\right)^T\right)\right]$, as a result, in order to avoid gradient vanishing or explosion, it's better to have $E\left[eig\left(\left(\mathbf{J_j}\mathbf{J_j}\right)^T\right)\right]\approx1$.




\eqref{equ:expectation_of_singular_equ} shows that as long as the $E[[\mathbf{\Sigma}]^2_i] \approx 1$, the difference will be neither scaled up exponentially nor decayed. $E[[\mathbf{\Sigma}]^2_i]$ can be easily obtained through 
\begin{equation}
    E[[\mathbf{\Sigma}]^2_i] = E[eig(\mathbf{\widetilde{\Lambda}}_t\mathbf{\widetilde{\Lambda}}_t^T)] = \lim_{n\rightarrow \infty}\frac{1}{n}Tr(\mathbf{\widetilde{\Lambda}}_t\mathbf{\widetilde{\Lambda}}_t^T) \approx 1
\label{equ:target_E}
\end{equation}

A stronger version of \eqref{equ:target_E} is called \textit{Dynamical Isometry} \citep{saxe2013exact}, which requires all the singular value of the input-output jacobian concentrating near 1, or 
\begin{equation}
    D\left[eig(\mathbf{\widetilde{\Lambda}}_t\mathbf{\widetilde{\Lambda}}_t^T)\right] = \lim_{n\rightarrow \infty}\frac{1}{n}Tr\left((\mathbf{\widetilde{\Lambda}}_t\mathbf{\widetilde{\Lambda}}_t^T)^2\right) - \left(E[eig(\mathbf{\widetilde{\Lambda}}_t\mathbf{\widetilde{\Lambda}}_t^T)]\right)^2 \approx 0
\label{equ:target_V}
\end{equation}

In the rest part of this paper, we use \eqref{equ:target_E} and \eqref{equ:target_V} as two metrics of the neural network.
\end{comment}

==> chapters/theoretical_discussion.tex <==



==> chapters/well_behaved_network.tex <==
\subsection{Continue the derivation in Sec. \ref{sec:dynaimc_of_}}
For neural networks that whose $\phi(\mathbf{JJ}^T)$ can be break down with \textbf{Theorem \ref{theorem:multiplication}}, we have
\begin{equation}
\begin{split}
    & E\left[||\mathbf{\delta_L}||_2^2\right] = \Pi_{i=1}^LE[tr(\mathbf{J_iJ_i}^T)]E\left[||\mathbf{\delta_0}||_2^2\right]\\
    & E[||\Delta \mathbf{\theta_i}||_2^2] = \eta^2\Pi_{j=1+1}^LE[tr(\mathbf{J_jJ_j}^T)]E[tr(\left(\frac{\partial \mathbf{f_{i}}}{\partial \mathbf{\theta_{i}}}\right)^T\frac{\partial \mathbf{f_{i}}}{\partial \mathbf{\theta_{i}}})]E[||\mathbf{x}||_2^2]
\end{split}
\label{equ:for_back_l2norm}
\end{equation}
Inspired by which, we give the following proposition:
\begin{prop}
(Well-behaved Neural Network) A neural network is well-behaved if for any its blocks whose input-output jacobian is denoted as $\mathbf{J_i}$, $E[tr(\mathbf{J_iJ_i}^T)]\approx 1$.
\end{prop}





==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> style/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************

